XaaS: Acceleration as a Service to Enable Productive High-Performance Cloud Computing

HPC and Cloud have evolved independently, specializing their innovations into performance or productivity. Acceleration as a Service (XaaS) is a recipe to empower both fields with a shared execution platform that provides transparent access to computing resources, regardless of the underlying cloud or HPC service provider. Bridging HPC and cloud advancements, XaaS presents a unified architecture built on performance-portable containers. Our converged model concentrates on low-overhead, high-performance communication and computing, targeting resource-intensive workloads from climate simulations to machine learning. XaaS lifts the restricted allocation model of Function-as-a-Service (FaaS), allowing users to benefit from the flexibility and efficient resource utilization of serverless while supporting long-running and performance-sensitive workloads from HPC.

==> references.tex <==
\begin{thebibliography}{1}

\bibitem{AA1}
J. J. Dongarra, I. S. Duff, D. C. Sorensen, H. A. van der Vorst,
\emph{Numerical Linear Algebra for High-Performance Computers}. SIAM 1998.

%\bibitem{BB2}
%T. Yeh, H. Chen, J. Chou, \emph{KubeShare: A Framework to Manage GPUs as First-Class and Shared Resources in Container Cloud}. HPDC 2020.

\bibitem{CC1}
M. AbdelBaky et al., \emph{Enabling High-Performance Computing as a Service}, in Computer, vol. 45, no. 10, pp. 72-80, Oct. 2012.

%\bibitem{DD1}
%L. Benedicic, F. A. Cruz, A. Madonna, K. Mariotti, \emph{Sarus: Highly Scalable Docker Containers for HPC Systems}. ISC High Performance 2019.

\bibitem{EE1}
M. Copik, K. Taranov, A. Calotoiu and T. Hoefler, \emph{rFaaS: Enabling High Performance Serverless with RDMA and Leases}. IPDPS 2023.

\bibitem{FF1}
I. Foster, \emph{Globus Online: Accelerating and Democratizing Science through Cloud-Based Services}, in IEEE Internet Computing, vol. 15, no. 3, pp. 70-73, May-June 2011.

\bibitem{GG1}
M. Armbrust, \emph{Above the Clouds: A Berkeley View of Cloud Computing}, Technical Report No. UCB/EECS-2009-28. URL: \url{https://www2.eecs.berkeley.edu/Pubs/TechRpts/2009/EECS-2009-28.pdf}

\bibitem{HH1}
I. Foster, Y. Zhao, I. Raicu and S. Lu, \emph{Cloud Computing and Grid Computing 360-Degree Compared}. 2008 Grid Computing Environments Workshop, 2008.

%\bibitem{II1}
%I. Foster, D. B. Gannon, \emph{Cloud Computing for Science and Engineering}. MIT Press 2017.

\bibitem{OO1}
W. Qiu, M. Copik, Y. Wang, A. Calotoiu, T. Hoefler, \emph{User-guided Page Merging for Memory Deduplication in Serverless Systems}, IEEE Big Data 2023.

\bibitem{II2}
N. Brown, et al., \emph{Utilising urgent computing to tackle the spread of mosquito-borne diseases}. 2021 IEEE/ACM HPC for Urgent Decision Making (UrgentHPC).

%\bibitem{MM2}
%T. Goubier, N. Rakowsky and S. Harig, \emph{Fast Tsunami Simulations for a Real-Time Emergency Response Flow}. 2020 IEEE/ACM HPC for Urgent Decision Making (UrgentHPC).

%\bibitem{NN2}
%A. Kremin, S. Bailey, J. Guy, T. Kisner and K. Zhang, \emph{Rapid Processing of Astronomical Data for the Dark Energy Spectroscopic Instrument}. 2020 IEEE/ACM HPC for Urgent Decision Making (UrgentHPC).

\bibitem{OO2}
R. Vescovi et al., \emph{Linking scientific instruments and computation: Patterns, technologies, and experiences}. Patterns, Volume 3, Issue 10, 2022.

\bibitem{OO2}
K. P. Keegan, E. M. Glass, F. Meyer, \emph{MG-RAST, a Metagenomics Service for Analysis of Microbial Community Structure and Function}. Methods in Molecular Biology, vol 1399, pp. 207-233, 2016.

\bibitem{OO3}
T. Hoefler et al., \emph{Earth Virtualization Engines: A Technical Perspective}, in Computing in Science \& Engineering, vol. 25, no. 3, pp. 50-59, May-June 2023.

\bibitem{OO4}
T. Ben-Nun, J. de Fine Licht, A. N. Ziogas, T. Schneider, T. Hoefler, \emph{Stateful dataflow multigraphs: a data-centric model for performance portability on heterogeneous architectures}. SC 2019.

\end{thebibliography}

